Any2Any: Incomplete Multimodal Retrieval with Conformal Prediction

Autonomous agents perceive and interpret their surroundings by integrating multimodal inputs, such as vision, audio, and LiDAR. These perceptual modalities support retrieval tasks, such as place recognition in robotics. However, current multimodal retrieval systems encounter difficulties when parts of the data are missing due to sensor failures or inaccessibility, such as silent videos or LiDAR scans lacking RGB information. We propose Any2Any-a novel retrieval framework that addresses scenarios where both query and reference instances have incomplete modalities. Unlike previous methods limited to the imputation of two modalities, Any2Any handles any number of modalities without training generative models. It calculates pairwise similarities with cross-modal encoders and employs a two-stage calibration process with conformal prediction to align the similarities. Any2Any enables effective retrieval across multimodal datasets, e.g., text-LiDAR and text-time series. It achieves a Recall@5 of 35% on the KITTI dataset, which is on par with baseline models with complete modalities.

==> figure_latex/clap_results.tex <==
\begin{table*}[t!]
    \centering
    \small
    \begin{tabular}{cccccccc}\hline
    Dataset & Method & mAP@$5$ & Precision@$1$ & Precision@$5$ & Precision@$20$ & Recall@$5$ & Recall@$20$ \\ \hline\hline
    MSR-VTT & Any2Any Incomplete & $8.5\%$ & $26.8\%$ & $11.0\%$ & $3.7\%$ & $42.5\%$ & $55.0\%$ \\
    (CLIP+CLAP) & Any2Any Complete  & $10.8\%$ & $30.5\%$ & $13.7\%$ & $4.8\%$ & $48.3\%$ & $64.0\%$ \\
    \hline
    \end{tabular}
    \captionof{table}{\small{\textbf{Any2Any retrieval results:}
    The results are similar to \Tabref{table:results}, showcasing that the Any2Any framework can work with any embeddings from any encoders.
    }}
    \label{table:clap}
    \vspace{-1em}
\end{table*}

==> section/acknowledgement.tex <==
We thank Sai Shankar Narasimhan and Pulkit Paliwal for providing insights on the time series retrieval task.
